Rethinking Intersection Over Union for Small Object Detection in Few-Shot Regime

In Few-Shot Object Detection (FSOD), detecting small objects is extremely difficult. The limited supervision cripples the localization capabilities of the models and a few pixels shift can dramatically reduce the Intersection over Union (IoU) between the ground truth and predicted boxes for small objects. To this end, we propose Scale-adaptive Intersection over Union (SIoU), a novel box similarity measure. SIoU changes with the objects' size, it is more lenient with small object shifts. We conducted a user study and SIoU better aligns than IoU with human judgment. Employing SIoU as an evaluation criterion helps to build more user-oriented models. SIoU can also be used as a loss function to prioritize small objects during training, outperforming existing loss functions. SIoU improves small object detection in the non-few-shot regime, but this setting is unrealistic in the industry as annotated detection datasets are often too expensive to acquire. Hence, our experiments mainly focus on the few-shot regime to demonstrate the superiority and versatility of SIoU loss. SIoU improves significantly FSOD performance on small objects in both natural (Pascal VOC and COCO datasets) and aerial images (DOTA and DIOR). In aerial imagery, small objects are critical and SIoU loss achieves new state-of-the-art FSOD on DOTA and DIOR.

==> Parts/01_introduction_old.tex <==
\section{Introduction}
\label{sec:intro}

Intersection over Union (IoU), also known as Jaccard index, is a well-known
similarity measure between sets. Besides its application in statistics, it is
widely used in computer vision to assess the quality of visual tasks such as
detection (\eg \cite{ren2015faster,redmon2016you, liu2016ssd}) and segmentation (\eg
\cite{long2015fcn, ronneberger2015convolutional, he2017mask}). The goal of
these tasks is to find sets of pixels that belong to a certain object or class.
The IoU can compute how close two sets of pixels are and therefore gives a
similarity measure between ground truth and the proposition of a model. In this
paper, we focus mainly on the detection task, although our propositions could be
applied to segmentation or any task that already use IoU. 
In detection, objects are localized using rectangular bounding boxes. IoU
therefore measures how much two bounding boxes overlap. 

IoU has a remarkable property: scale invariance. It means that if two bounding
boxes have a certain IoU, scaling both boxes by the same amount will not change
the IoU.
% (provided that the shift between boxes is scaled as well).
At first glance, this seems a desirable property, all objects will be treated
identically no matter their size. In practice, it has a fundamental drawback:
small boxes are prone to large IoU changes from only small position or size
modification. To clarify this issue, let us consider a simple example. Two
square boxes of width $\omega$ are shifted horizontally by $\rho$ pixels. In
this setup increasing the shift by 1 pixel leads to a slight decrease in IoU.
This reduction will be larger if the boxes are small. This comes from the scale
invariance property as IoU stays constant as the ratio $\frac{\rho}{\omega}$
is constant. However, this ratio varies quicker for small objects, causing quick
IoU drops for only few pixels inaccuracies as shown in \cref{fig:pixel_shift}.
This is problematic because a box shifted only a few pixels from the ground
truth can fall under the IoU threshold and be considered as a false detection.
We show this behavior in \cref{sec:shift_analysis,sec:inaccuracy}, which explore
the resilience of various criteria to pixel shifts and localization inaccuracies
respectively. Nevertheless, slightly shifted boxes are still considered
satisfactory detections from a human perspective (see \cref{sec:user_study}).
Therefore, IoU is not an optimal box similarity measure for evaluation as it
does not fully align with human perception. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/iou_vs_siou_same_mod.png}
    \caption{Evolution of various criteria (IoU, NWD, SIoU and $\alpha$-IoU)
    when a box is shifted from the ground truth box by $\rho$ pixels for
    various box sizes (4, 16, 64, 128). On the \textbf{left}, both
    boxes have the same size, on the \textbf{right} ground truth is $1.25$
    larger.}
    \label{fig:pixel_shift}
\end{figure}

The difficulty of detecting small objects was reported in many object detectors
\cite{ren2015faster,redmon2016you, liu2016ssd,
tian2019fcos,duan2019centernet,law2018cornernet,carion2020end}. Numerous
attempts have been made to fill this shortcoming by proposing pyramidal features
\cite{liu2016ssd, lin2017feature, zhang2018single } or  multiscale training
\cite{singh2018sniper, singh2021scale}, providing significant improvements.
However, this difficulty intensifies in the few-shot regime as shown by
\cite{lejeune2022improving}. When only few examples are available for each
class, finding small targets becomes even harder as the examples are small as
well. It is difficult to extract useful information from them and condition well
the detection toward the desired classes. Nevertheless, most detection methods
use IoU extensively as: a regression loss \cite{yu2016unitbox, tian2019fcos}; an
example selection criterion \cite{ren2015faster,redmon2016you, liu2016ssd}; a
criterion to filter output (through non-maximal suppression); or an evaluation
measure. Only a handful of works actually question the adequation of IoU for
object detection. Among those, \cite{rezatofighi2019generalized} proposed a
generalization of IoU when intersection between boxes is empty,
\cite{wang2021nwd} introduced a novel loss function to target small object
specifically and \cite{strafforello2022humans} showed that human perception and
IoU are not completely aligned.

In this paper, we revisit Intersection over Union to improve Few-Shot Object
Detection (FSOD) methods and in particular their application on aerial imagery.
Small object detection is already problematic with natural images, but it is
reinforced in the few-shot regime and on aerial images. To this end, we propose
Scale-adaptive Intersection over Union (SIoU), a novel criterion that can be used just
as IoU for training and evaluating detection models. To demonstrate the
superiority of the proposed SIoU, \cref{sec:criterion_analysis} compares it with
various existing criteria. This section analyzes the criteria's distributions
when they are exposed to randomly shifted boxes. This study helps to understand
what makes a better criterion for performance evaluation. To our knowledge, this
is the first attempt to study empirically and theoretically the distributions of
these criteria. The conclusions of this analysis are then compared with human
perception through a user study which shows that SIoU aligns better with human
evaluation than IoU (see \cref{sec:user_study}). The comparison of the criteria
also highlights that SIoU can guide training towards small objects better than
other criteria and in more controlled fashion. SIoU can be tuned to improve the
detection of small objects just as it can be tuned to align with human
perception. Finally, this is confirmed by extensive experiments on both aerial
images (DOTA \cite{xia2018dota} and DIOR \cite{li2020dior}) and natural images
(Pascal VOC \cite{everingham2010pascal}. \\

\noindent
The main contributions of this paper are as follows:

\begin{itemize}[noitemsep]
    \item[-] A novel scale-adaptive criterion called SIoU that can be tuned for detecting
    objects of various sizes.% and which outperforms existing criteria. 
    \item[-] An empirical and theoretical analysis of the distributions of existing
    criteria that helps to understand required properties for designing
    regression loss function and evaluation criteria.
    \item[-] A user study that demonstrates the misalignment between IoU and human
    perception on the detection task.
    \item[-] Extensive experiments on various datasets to support the superiority of
    SIoU for detection small objects. 
\end{itemize}



==> Parts/02_existing_work_old.tex <==
\section{Related Works}
\label{sec:rel_work}

\subsection{Intersection over Union and its variants}
To begin, let us review the definition of existing criteria for set similarity.
First, the IoU or Jaccard index is defined as the
intersection area of two boxes divided by the area of their union: 

\begin{equation}
    \text{IoU}(A, B) = \frac{|A \cap B|}{|A \cup B|},
\end{equation}

\noindent
where $A$ and $B$ are two sets. When $A$ and $B$ are rectangular boxes, IoU can
be computed easily with simple operations on the boxes coordinates. This
explains why IoU is such a widespread criterion for object detection. It is used
as a loss function $\mathcal{L}_{\text{reg}} = 1 - \text{IoU}$ by a number of
well established detection framework (\eg \cite{yu2016unitbox, tian2019fcos}).
IoU is also involved in the processus of example selection during training of
most detection methods, basically all methods inspired either by Faster R-CNN
\cite{ren2015faster} or YOLO \cite{redmon2016you}. In these frameworks,
regression loss is computed between coordinates of proposed boxes and ground
truth boxes. Not all pairs of proposals and ground truth are kept for the
computation. Only proposals with a sufficient IoU with a ground truth box are
selected. Finally, IoU is also used as the heart of the evaluation process. A
proposed box is considered as a positive detection if it meets two conditions:
1) has an IoU greater than a given threshold with a ground truth box and 2) has
the same label as this ground truth. 

Several attempts where made to modify IoU but existing works mostly focus on the
regression loss part, disregarding the others IoU involvements in the detection
task. First, \cite{rezatofighi2019generalized} proposed a generalized version of
IoU which yields negative values when boxes do not overlap: 
\begin{equation}
    \text{GIoU}(A,B) = \text{IoU}(A,B) - \frac{|C \backslash (A \cup B)|}{|C|},
\end{equation}

\noindent
where $C$ is the convex hull around $A$ and $B$. This criterion is employed as a
loss function by several detection frameworks \cite{tian2019fcos,
bochkovskiy2020yolov4, zhang2020bridging}. It is sometimes also combined with
other regression loss as in \cite{li2020generalized, carion2020end}, which both
combine it with a L1 regression on boxes coordinates. Combining IoU loss with
more standard regression losses was also proposed by \cite{zheng2020distance}.
They introduce two losses Distance-IoU (DIoU) and Complete-IoU which
respectively add a L2 regression term and an aspect ratio penalty to the IoU
loss. Recently, $\alpha$-IoU \cite{he2021alpha} extends DIoU
\cite{zheng2020distance} by proposing a family of losses following the same
structure as DIoU with the IoU term raised to the power $\alpha$. Alternatively,
Bounded IoU \cite{tychsen2018improving} computes an IoU upper bound between a
proposal and a ground truth. 

All previous IoU improvements were made to tackle the regression part of the
models. However, IoU is involved in other part of the framework including
example selection, non-maximal suppression (NMS) and evaluation. A recent user
study conducted in \cite{strafforello2022humans} indicates that IoU does not
completely align with human perception. Humans tend to prefer larger boxes over
smaller one at constant IoU with a ground truth box. This suggests that IoU is
not an optimal choice either in example selection nor in evaluation as it will
lead to detections that do not statisfy human users.  

\subsection{Object Detection}
Object Detection is a problem that has been studied for decades. It witnessed
rapid progress with the rise of deep learning methods
\cite{ren2015faster,redmon2016you, liu2016ssd}. Recent methods achieve very
satisfactory results when provided with sufficient data. However, there remains
some challenges to master object detection. Most object detectors still
struggle with small objects and when data is scarce. \\


\noindent
\textbf{Small Object Detection} is a challenging task and while there has been
plenty of attemps to improve it based on pyramidal features \cite{liu2016ssd,
lin2017feature, zhang2018single }, multiscale training \cite{singh2018sniper,
singh2021scale}, data-augmentation \cite{kisantal2019augmentation} or
super-resolution \cite{rabbi2020small, Bai2018SODMTGANSO, Shermeyer2019TheEO,
Courtrai2020SmallOD,Ferdous2019SuperRD}. Only few works actually tackle this
problem by changing the loss function. Normalized Wasserstein Distance
\cite{wang2021nwd} (NWD) proposes an alternative to IoU specifically designed
for detecting small objects. It consists of computing the Wasserstein distance
between two gaussian distributions fitted on the two bounding boxes compared.
Moreover, NWD is not only used as a loss function but also as an example
selection criterion.\\


\noindent
\textbf{Few-Shot Object Detection (FSOD)} is the task of detecting objects only
provided a handful of examples per class. Specifically, $N$-way $K$-shot object
detection consists in detecting objects belonging to a set of $N$ classes with
only $K$ annotated images for each class. Many approaches were proposed in the
literature to address this problem: metric learning
\cite{karlinsky2019repmet,yang2020restoring, sun2021fsce, jeune2021experience},
simple fine-tuning \cite{chen2018lstd, wang2020frustratingly, wolf2021double,
xu2022simpl} and attention-based methods \cite{kang2019few, xiao2020fsod,
han2021meta, zhang2021meta, chen2021should}. The similarity between all these
works is that they learn generic knowledge from a set of \textit{base classes}
with plenty of annotations and adapt to \textit{novel classes} from the few
available examples. Recently, it has been shown \cite{lejeune2022improving} that
FSOD is even more sensitive to small objects than regular object detection.
Extracting information from small object is hard and produces spurious features
that do not condition well the detection. Some solutions are proposed to
overcome with augmentation and careful example cropping
\cite{lejeune2022improving} or with dedicated attention mechanisms
\cite{lejeune2022aaf}. Nevertheless, this is not enough to solve the issue of
small objects in FSOD. 

% In the following sections, we provide some orthogonal
% solutions based on a tunable criterion to replace IoU and prove its usefulness
% on FSOD. But it could very well be applied to regular object detection and other
% similar tasks such as segmentation.







